Reactive Synthesis: Branching Logics and Parameterized Systems

Reactive synthesis is an automatic way to translate a human intention expressed in some logic into a system of some kind. This thesis has two parts, devoted to logic and to systems. In Part I, we develop two new approaches to CTL* synthesis. The first approach consists of two extensions of the SMT-based bounded synthesis: one follows bottom-up CTL* model checking, another one follows the automata framework. The second approach reduces CTL* synthesis to LTL synthesis. The reduction turns any LTL synthesiser into a CTL* synthesiser. The two approaches were implemented and are available online. In Part II, we study parameterized synthesis for two system architectures. The first architecture is guarded systems and is inspired by cache coherence protocols. In guarded systems, processes transitions are enabled or disabled depending on the existence of other processes in certain local states. The existing cutoff results for guarded protocols are restricted to closed systems, and are of limited use for liveness properties. We close these gaps and prove tight cutoffs for open systems with liveness properties, and also cutoffs for detecting deadlocks. The second architecture is token-ring systems, where the single token circulates processes arranged in a ring. The experiments with the existing parameterized synthesis method showed that it does not scale to large specifications. First, we optimize the method by refining the cutoff reduction, using modularity and abstraction. The evaluation show several orders of magnitude speed-ups. Second, we perform parameterized synthesis case study on the industrial arbiter protocol AMBA. We describe new tricks ---a new cutoff extension and decompositional synthesis--- that, together with the previously described optimizations, allowed us to synthesize AMBA in a parameterized setting, for the first time.

==> guarded-systems/experiments.tex <==
\section{Experiments} \label{gua:sec:experiments}

(The experiments were done by S. Au{\ss}erlechner,
 as a part of his Master Thesis.)

We used our new cutoff results in the context of parameterized synthesis to 
automatically construct process templates with safety and liveness guarantees 
for guarded systems with an arbitrary number of components.
Our prototype is an extension of the parameterized synthesis tool 
{\sc Party}~\cite{party}.
It synthesizes process templates based on the semi-decision procedure 
described in Section~\ref{gua:sec:paramsynt}. 
Bounded template synthesis is 
implemented as an extension of the bounded synthesis approach~\cite{BS}, with
LTL3BA~\cite{LTL3BA} for translation of specifications to automata, and
SMT solver Z3~\cite{Moura08} as backend. 

%In the cutoff detection step, we apply the cutoff results from 
%Section~\ref{gua:sec:cutoffs} modularly, i.e., we calculate cutoffs and convert 
%to universal co-Büchi tree automaton (UCT)\sj{remind/use long version} for every conjunct of the specification separately (an optimization 
%mentioned in~\cite{KhalimovJB13b}). Finally, we produce the SMT encoding, 
%conjoining the SMT constraints for all parts. 
%
As a proof of concept, we synthesized implementations for two small 
examples (on a single core of a 3.5GHz Intel i7 CPU with 4GB RAM):
\begin{itemize}
\item a closed disjunctive system $\largesys$ where $A$ controls an output 
signal $w$, and every $B_i$ a signal $g_i$, with fairness assumption and specification
$\GF(\neg w) \wedge \GF w \wedge 
\bigwedge_{i} \left[\GF(w \wedge g_i) \wedge  \GF g_i \wedge \GF(\neg g_i) 
\right]$,
i.e., all processes must toggle their signals 
infinitely often, and every process $B^i$ must ``meet'' infinitely often with 
$A$ when both signals are enabled. The implementation below has been synthesized with a cutoff of $2\card{B}+1-1=4$ for the property and $2\card{B}-1=3$ for the deadlock detection within one minute.

\item an open conjunctive system $(B)^{(n)}$ (i.e., $A$ can be arbitrary and $B$ does not react to it), where each process $B_i$ gets requests of high and low priority as input ($rh_i, rl_i$), and controls ouputs that represent grants to these requests ($gh_i, gl_i$). The specification requires i) `every request $rh$ should eventually be granted ($gh_i$)', ii) `every request $rl_i$ should eventually be granted ($gl_i$) unless there is a simultaneous request $rh_i$', iii) `there should be no spurious grants', iv) `mutual exclusion of grants (locally and globally)'. The implementation above has been synthesized with a cutoff of $3$ for properties, and $4$ for deadlock detection within about $45$ minutes. Note that we do not restrict the implementation to $1$-conjunctive systems, and therefore the cutoff does not guarantee absence of local deadlocks in systems of arbitrary size.
\end{itemize}

\begin{figure}[ptb]
\centering
\begin{subfigure}[b]{0.45\textwidth}\center
\scalebox{0.7}{\input{guarded-systems/img/disjunctive_lts}}
\caption{Disjunctive system}
\label{fig:disjunctiveLTS}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}\center
\scalebox{0.7}{\input{guarded-systems/img/mutual_exclusion3_lts}}
\label{fig:conjunctiveLTS3}
% \caption{Templates $(A,B)$ used to prove the tightness of the cutoffs for properties $\pexists h(A^1,B^1)$ (Observation~\ref{obs:disj:tight_prop})\ak{check me}.}
\label{fig:experiments}
\caption{Conjunctive system}
\end{subfigure}
\caption{Synthesized systems}
\end{figure}


==> guarded-systems/img/conj_deadlock_cutoff.tex <==
\begin{tikzLTS}
      \tikzstyle{state} = [circle,draw=black,thick,inner sep=1.5pt, text width={width("$\text{T}_{i-1}$")}, align=center]
      \tikzstyle{boxLabel} = [yshift=-0.4cm]
      \tikzstyle{every node} = [node distance=3cm]

  \node[state] (A) [] {$\text{init}$};
  \node[] (B) [below of=A, node distance=2.5cm] {$$};
  \node[state] (C) [left of=B, node distance=3.5cm] {$1$};
  \node[state] (D) [right of=C] {$2$};
  \node[] (B) [below of=A] {$$};
  \node[] (E) [right of=D] {$$};
  \node[] (E') [below of=E,node distance=0.75cm] {$$};
  \node[node distance=1cm] (F) [right of=E] {$$};
  \node[state] (G) [right of=F] {$n$};
  
\pgfmathsetmacro{\shift}{0.3ex}

\draw [post] (A.185) -- node[above] {} (C.80);
\draw [pre] (A.210) -- node[below right] {$\neg 1$} (C.55);

\draw [post] (A.245) -- node[above] {} (D.90);
\draw [pre] (A.270) -- node[below right] {$\neg 2$} (D.65);

\draw [post] (A.325) -- node[above] {} (G.150);
\draw [pre] (A.350) -- node[above right] {$\neg n$} (G.125);
  
  \path (C) edge [right,post] node [above] {$\neg 2$} (D);
  \path (D) edge [right,post] node [above] {$\neg 3$} (E);
  \path ($(E)-(0.05,0)$) edge [right,dotted,-] node [above] {} ($(F)+(0.05,0)$);
  \path (F) edge [right,post] node [above] {$\neg n$} (G);
  
  \path (G) edge [bend left,post] node [above] {$\neg 1$} (C);
  
   \node (U2) [draw=black, fit=(A) (C) (G) (E'), inner sep=0.75cm] {};
   \node [boxLabel] at (U2.north) {Template $B$};
\end{tikzLTS}

==> guarded-systems/img/disj_tight_propA_tmplA.tex <==
%!TEX root = table.tex
\begin{tikzpicture}[node distance=2cm,inner sep=1pt,minimum size=0.5mm,->,>=latex]


\node[state,double] (a_1) {$a_1$};
\node (dots) [right of=a_1] {$\ldots$};
\node[state] (a_n) [right of=dots] {$a_{all}$};


\path (a_1) edge [above] node {$\disj{b_1}$} (dots);
\path (dots) edge [above] node {$\disj{b_{|T_B|}}$} (a_n);



\end{tikzpicture}


==> guarded-systems/img/disj_tightness_fair_prop.tex <==
\begin{tikzLTS}
      \tikzstyle{state} = [circle,draw=black,thick,inner sep=1.5pt, text width={width("$\text{init}_1$")}, align=center]
      \tikzstyle{boxLabel} = [yshift=-0.4cm]

    \newcommand{\rad}{2 }
    \draw[draw=white] (0,0) circle (3);
    \foreach \x[remember=\x as \lastx] in {1,2,...,5}{
      \ifnum \x < 4
      \node[state] (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) {$a_\x$};
      \else
       \ifnum \x = 4
         \coordinate (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) ;
        \else
         \node[state] (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) {$a_{|T_B|}$};
        \fi
      \fi
    }

    \coordinate (t34) at ($(0,0)+({-72*(4-2)+36}:\rad and \rad)$) ;
    \coordinate (t44) at ($(0,0)+({-72*(4-2)-0}:\rad and \rad)$) ;

      \path (t1) [post,bend left] edge node[above right] {$\disj{b_1}$} (t2);
      \path (t2) [post,bend left] edge node[below right] {$\disj{b_2}$} (t3);
      \path (t3) [post,bend left,dashed] edge node[below] {$\disj{b_3}$} (t34);
      \path (t34) [bend left,dotted] edge (t44);
      \path (t44) [post,bend left,dashed] edge node[above right] (e34-44) {$\disj{b_{|T_B|-1}}$} (t5);
      \path (t5) [post,bend left] edge node[above left] {\disj{b_{|T_B|}}} (t1);

	 \node (U1) [draw=black, fit=(t1) (t2) (t3) (t4) (t5) (t34) (t44), inner sep=0.75cm] {} ;
	 \node [boxLabel] at (U1.north) {Template $A$};

     \coordinate(tright) at (U1.east);
     %\draw[black] ($(t5.west |- t1.north)-(1, -1)$) rectangle ($(t2.east |- t3.south)+(1,-1)$);
     %\path  ($(t5.west |- t1.north)-(1, -1.1)$) -- ($(t2.east |- t1.north)+(1, 1.1)$) node[midway,above] {$\mathcal{T}_1$};

    \newcommand{\dist}{4 }
    \node[state] (t1) at ($(tright |- t1)+(4,0)$) {$b_1$};
    \node[state] (t2) at ($(tright |- t3)+(\dist/2,0.5)$) {$b_2$};
    \node[state] (t3) at ($(tright |- t3)+(\dist/2+2,0.5)$) {$b_3$};
    \node (ti) at ($(tright |- t3)+(\dist/2+3.5,0)$) {\dots\dots};
    \node[state] (t5) at ($(tright |- t3)+(\dist/2+5,0)$) {$b_k$};

    \path (t1) edge[post,loop left] node[left] {\disj{b_1}} (t1)
              (t1) edge[post]  (t2)
              (t1) edge[post]  (t3)
              (t1) edge[post]  (t5)
%               (t1) edge[post] node[above left] {$|T_B|$} (t2)
%               (t1) edge[post] node[above right] {$|T_B|$} (t3)
%               (t1) edge[post] node[above right] {$|T_B|$} (t5)
              (t2) edge[post,loop below] node[below] {\disj{b_2}} (t2)
              (t3) edge[post,loop below] node[below] {\disj{b_3}} (t3)
              (t5) edge[post,loop below] node[below] {\disj{b_k}} (t5);

	 \coordinate(U1bottom) at ($(t2 |- U1.south)+(0,0.75)$);
     \node (U2) [draw=black, fit=(t1) (t2) (t3) (ti) (t5) (U1bottom), inner sep=0.75cm] {} ;
	 \node [boxLabel] at (U2.north) {Template $B$};;



\end{tikzLTS}

==> guarded-systems/img/disj_tightness_fair_prop_run.tex <==
\begin{tikzPath}    
    \node (T21-0) [pstate,label=right:$a_1$] {}; 
    \node (T21-1) [below of=T21-0,hiddenstate,label=right:$$] {};           
    \node (T21-2) [below of=T21-1,pstate,label=right:$a_1$] {};
    \node (T21-3) [below of=T21-2,pstate,label=right:$a_2$] {};           
    \node (T21-4) [below of=T21-3,pstate,label=right:$a_3$] {};
    \node (T21-5) [below of=T21-4,hiddenstate,label=right:$$] {};
        
    \draw[trans-notsched,dashed] (T21-0) -- (T21-2); 
    \draw[trans-notsched] (T21-2) -- (T21-3);
    \draw[trans-notsched] (T21-3) -- (T21-4);
    \draw[trans-notsched] (T21-4) -- (T21-5);
    
    \node (T22-0) [pstate,right of=T21-0,label=right:$b_1$,node distance=1cm] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};           
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched,dashed] (T22-0) -- (T22-5);
    
    \node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=1cm] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};           
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched,dashed] (T22-0) -- (T22-5);

\newcommand{\patht}[2]{
    \node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=#1] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,pstate,label=right:$#2$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};    
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched] (T22-0) -- (T22-2);
    \draw[trans-notsched,dashed] (T22-2) -- (T22-5);
}

    \patht{1cm}{b_1}
    \patht{1cm}{b_2}
    \patht{1cm}{b_2}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots$,node distance=0.75cm] {}; 
    \patht{1.5cm}{b_{|T_B|}}
    \patht{1cm}{b_{|T_B|}}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots\dots$,node distance=1cm] {}; 
    \end{tikzPath}

==> guarded-systems/img/fig_conj_deadlock-detection-worst-impl.tex <==
\begin{tikzLTS}
      \tikzstyle{state} = [circle,draw=black,thick,inner sep=1.5pt, text width={width("$\text{T}_{i-1}$")}, align=center]
      \tikzstyle{boxLabel} = [yshift=-0.4cm]
      \tikzstyle{every node} = [node distance=3cm]
    
    \node[] (ti) {$\dots\dots\dots\dots$};
    
    \node[state] (t3) [left of=ti, node distance=2cm] {$b_3$};
    \node[state] (t2) [left of=t3] {$b_2$};
    \node[state] (t4) [right of=ti, node distance=2cm] {$b_{i-1}$};
    \node[state] (t5) [right of=t4] {$b_i$};
    \node[] (tii) [right of=t5, node distance=1.5cm] {$\dots\dots$};

    \node[state] (t1) [above of=ti] {$b_1$};


	\draw (t1) [post, bend right] edge node [above left] (l1) {} (t2);
	\draw (t1) [post] edge node [above left] (l1) {} (t3);
	\draw (t1) [post] edge node [above right] (l1) {} (t4);
	\draw (t1) [post, bend left] edge node [above right] (l1) {} (t5);
	
	\draw (t2) [post, loop above] edge node [above] {$\forall{\neg b_2}$} (t2);
	
	\draw (t2) [post, bend left] edge node [above] {$\forall{\neg b_3}$} (t3);
	\draw (t3) [post, bend left] edge node [below] {$\forall{\neg b_3}$} (t2);
	
	\draw (t4) [post, bend left] edge node [above] {$\forall{\neg b_i}$} (t5);
	\draw (t5) [post, bend left] edge node [below] {$\forall{\neg b_i}$} (t4);

 	 \node (U2) [draw=black, fit=(t1) (t2) (tii), inner sep=0.75cm] {};
 	 \node [boxLabel] at (U2.north) {Template $B$};
\end{tikzLTS}

==> guarded-systems/img/fig_conjunctive-deadlock-detection-impossible-comp.tex <==
\begin{tikzPath}	
     	\node (T21-0) [pstate,label=right:$a_1$] {}; 
     	\node (T21-1) [below of=T21-0,hiddenstate,label=right:$$] {};   		
     	\node (T21-2) [below of=T21-1,hiddenstate,label=right:$$] {};
     	\node (T21-3) [below of=T21-2,pstate,label=right:$a_1$] {};   		
	\node (T21-4) [below of=T21-3,pstate,label=right:$a_1$] {};
	    
	\draw[trans-notsched,dashed] (T21-0) -- (T21-3); 
	\draw[trans-notsched] (T21-3) -- (T21-4);
	
     	\node (T22-0) [pstate,right of=T21-0,label=right:$b_1$,node distance=1cm] {}; 
     	\node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};   		
     	\node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
     	\node (T22-3) [below of=T22-2,pstate,label=right:$b_1$] {};   		
     	\node (T22-4) [below of=T22-3,pstate,label=right:$b_1$] {};

	\draw[trans-notsched,dashed] (T22-0) -- (T22-3);
	\draw[trans-notsched] (T22-3) -- (T22-4);

\newcommand{\patht}[3]{
     	\node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=#1] {}; 
     	\node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};   		
     	\node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
     	\node (T22-3) [below of=T22-2,pstate,label=right:$#2$] {};
	\node (T22-4) [below of=T22-3,pstate,label=right:$#3$] {};

	\draw[trans-notsched] (T22-0) -- (T22-3);
	\draw[trans-notsched] (T22-3) -- (T22-4);
}

    \patht{1cm}{a_1}{a_1}
    \patht{1cm}{b_2}{b_2}
    \patht{1cm}{b_2}{b_2}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots\dots$,node distance=1cm] {}; 
    \patht{2cm}{b_d}{b_d}
    \patht{1cm}{b_d}{b_d}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots\dots$,node distance=1cm] {}; 
    \patht{2cm}{b_{|T_B|}}{b_{|T_B|}}
    \patht{1cm}{b_d}{b_{|T_B|}}
    \end{tikzPath}

==> guarded-systems/img/fig_disj-bounding_worst-comp.tex <==
\begin{tikzPath}    
    \node (T21-0) [pstate,label=right:$a_1$] {}; 
    \node (T21-1) [below of=T21-0,hiddenstate,label=right:$$] {};           
    \node (T21-2) [below of=T21-1,pstate,label=right:$a_1$] {};
    \node (T21-3) [below of=T21-2,pstate,label=right:$a_2$] {};           
    \node (T21-4) [below of=T21-3,pstate,label=right:$a_3$] {};
    \node (T21-5) [below of=T21-4,hiddenstate,label=right:$$] {};
        
    \draw[trans-notsched,dashed] (T21-0) -- (T21-2); 
    \draw[trans-notsched] (T21-2) -- (T21-3);
    \draw[trans-notsched] (T21-3) -- (T21-4);
    \draw[trans-notsched] (T21-4) -- (T21-5);
    
    \node (T22-0) [pstate,right of=T21-0,label=right:$b_1$,node distance=1cm] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};           
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched,dashed] (T22-0) -- (T22-5);
    
    \node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=1cm] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};           
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched,dashed] (T22-0) -- (T22-5);

\newcommand{\patht}[2]{
    \node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=#1] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,pstate,label=right:$#2$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};    
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched] (T22-0) -- (T22-2);
    \draw[trans-notsched,dashed] (T22-2) -- (T22-5);
}

    \patht{1cm}{b_1}
    \patht{1cm}{b_2}
    \patht{1cm}{b_2}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots$,node distance=0.75cm] {}; 
    \patht{1.5cm}{b_{|T_B|}}
    \patht{1cm}{b_{|T_B|}}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots\dots$,node distance=1cm] {}; 
    \end{tikzPath}

==> guarded-systems/img/fig_disj-bounding_worst-comp2.tex <==
\begin{tikzPath}    
    \node (T21-0) [pstate,label=right:$a_1$] {};    
    \node (T21-1) [below of=T21-0,hiddenstate,label=right:$$] {};           
    \node (T21-2) [below of=T21-1,hiddenstate,label=right:$$] {};
    \node (T21-3) [below of=T21-2,hiddenstate,label=right:$$] {};           
    \node (T21-4) [below of=T21-3,hiddenstate,label=right:$$] {};
    \node (T21-5) [below of=T21-4,hiddenstate,label=right:$$] {};
    \draw[trans-notsched,dotted] (T21-0) -- (T21-5);
            
    \node (T22-0) [pstate,right of=T21-0,label=right:$b_1$,node distance=1cm] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,pstate,label=right:$b_1$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};           
    \node (T22-4) [below of=T22-3,pstate,label=right:$b_{|T_B|}$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched,dashed] (T22-0) -- (T22-2);
    \draw[trans-notsched] (T22-2) -- (T22-4);
    \draw[trans-notsched,dashed] (T22-4) -- (T22-5);

\newcommand{\patht}[2]{
    \node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=#1] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,pstate,label=right:$#2$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};    
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched] (T22-0) -- (T22-2);
    \draw[trans-notsched,dashed] (T22-2) -- (T22-5);
}

    \patht{1cm}{b_1}
    \patht{1cm}{b_1}
    \patht{1cm}{b_2}
    \patht{1cm}{b_2}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots$,node distance=0.75cm] {}; 
    \patht{1.5cm}{b_{|T_B|}}
    %\node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots$,node distance=1cm] {}; 
    \end{tikzPath}

==> guarded-systems/img/fig_disj-bounding_worst-impl.tex <==
\begin{tikzLTS}
      \tikzstyle{state} = [circle,draw=black,thick,inner sep=1.5pt, text width={width("$\text{init}_1$")}, align=center]
      \tikzstyle{boxLabel} = [yshift=-0.4cm]
	  
    \newcommand{\rad}{2 }
    \draw[draw=white] (0,0) circle (3);
    \foreach \x[remember=\x as \lastx] in {1,2,...,5}{
      \ifnum \x < 4
      \node[state] (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) {$a_\x$};
      \else
       \ifnum \x = 4
         \coordinate (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) ;
        \else
         \node[state] (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) {$a_{|T_B|}$};
        \fi
      \fi
    }

    \coordinate (t34) at ($(0,0)+({-72*(4-2)+36}:\rad and \rad)$) ;
    \coordinate (t44) at ($(0,0)+({-72*(4-2)-0}:\rad and \rad)$) ;

      \path (t1) [post,bend left] edge node[above right] {$\disj{b_1}$} (t2);
      \path (t2) [post,bend left] edge node[below right] {$\disj{b_2}$} (t3);
      \path (t3) [post,bend left,dashed] edge node[below] {$\disj{b_3}$} (t34);
      \path (t34) [bend left,dotted] edge (t44);
      \path (t44) [post,bend left,dashed] edge node[above right] (e34-44) {$\disj{b_{|T_B|-1}}$} (t5);
      \path (t5) [post,bend left] edge node[above left] {\disj{b_{|T_B|}}} (t1);
      
	 \node (U1) [draw=black, fit=(t1) (t2) (t3) (t4) (t5) (t34) (t44), inner sep=0.75cm] {} ;
	 \node [boxLabel] at (U1.north) {Template $A$};
	 
     \coordinate(tright) at (U1.east);
     %\draw[black] ($(t5.west |- t1.north)-(1, -1)$) rectangle ($(t2.east |- t3.south)+(1,-1)$);
     %\path  ($(t5.west |- t1.north)-(1, -1.1)$) -- ($(t2.east |- t1.north)+(1, 1.1)$) node[midway,above] {$\mathcal{T}_1$};

    \newcommand{\dist}{4 }
    \node[state] (t1) at ($(tright |- t1)+(4,0)$) {$b_1$};
    \node[state] (t2) at ($(tright |- t3)+(\dist/2,0.5)$) {$b_2$};
    \node[state] (t3) at ($(tright |- t3)+(\dist/2+2,0.5)$) {$b_3$};
    \node (ti) at ($(tright |- t3)+(\dist/2+3.5,0)$) {\dots\dots};
    \node[state] (t5) at ($(tright |- t3)+(\dist/2+5,0)$) {$b_k$};
    
    \path (t1) edge[post,loop left] node[left] {\disj{b_1}} (t1)
              (t1) edge[post]  (t2)
              (t1) edge[post]  (t3)
              (t1) edge[post]  (t5)
%               (t1) edge[post] node[above left] {$|T_B|$} (t2)
%               (t1) edge[post] node[above right] {$|T_B|$} (t3)
%               (t1) edge[post] node[above right] {$|T_B|$} (t5)
              (t2) edge[post,loop below] node[below] {\disj{b_2}} (t2)
              (t3) edge[post,loop below] node[below] {\disj{b_3}} (t3)
              (t5) edge[post,loop below] node[below] {\disj{b_k}} (t5);
    
	 \coordinate(U1bottom) at ($(t2 |- U1.south)+(0,0.75)$);
     \node (U2) [draw=black, fit=(t1) (t2) (t3) (ti) (t5) (U1bottom), inner sep=0.75cm] {} ;
	 \node [boxLabel] at (U2.north) {Template $B$};;
     
  
      
\end{tikzLTS}

==> guarded-systems/img/fig_disj-bounding_worst-impl2.tex <==
\begin{tikzLTS}
      \tikzstyle{state} = [circle,draw=black,thick,inner sep=1.5pt, text width={width("$\text{init}_2$")}, align=center]
      \tikzstyle{boxLabel} = [yshift=-0.4cm]
      \tikzstyle{every node} = [node distance=1.75cm]
    
    \node[state] (t1) {$b_1$};
    \node[state] (t2) [below of=t1] {$b_2$};
    \node[] (t3) [below of=t2] {$$};
    \node[] (t4) [below of=t3, node distance=1cm] {$$};
    \node[state] (t5) [below of=t4] {$b_k$};




       \path (t1) [post,loop right] edge node [right] (l1) {$\disj{b_1}$} (t1);
       \path (t1) [post] edge node[right] {$\disj{b_1}$} (t2);
        \path (t2) [post,loop right] edge node [right] (l2) {$\disj{b_2}$} (t2);
        \path (t2) [post,dashed] edge node[right] {$\disj{b_2}$} (t3);
        \path (t3) [dotted] edge (t4);
        \path (t4) [post,dashed] edge node[right] {$\disj{b_{k-1}}$} (t5);
        \path (t5) [post,loop right] edge node[right] (l5) {$\disj{b_k}$} (t5);

  	 \node (U2) [draw=black, fit=(t1) (t2) (t3) (t4) (t5) (l1) (l2) (l5), inner sep=0.75cm] {} ;
 	 \node [boxLabel] at (U2.north) {Template $B$};
\end{tikzLTS}

==> macros.tex <==
\makeatletter
\if@titlepage
  \newenvironment{abstract}{%
      \titlepage
      \null\vfil
      \@beginparpenalty\@lowpenalty
      \begin{center}%
        \bfseries \abstractname
        \@endparpenalty\@M
      \end{center}}%
     {\par\vfil\null\endtitlepage}
\else
  \newenvironment{abstract}{%
      \if@twocolumn
        \section*{\abstractname}%
      \else
        \small
        \begin{center}%
          {\bfseries \abstractname\vspace{-.5em}\vspace{\z@}}%
        \end{center}%
        \quotation
      \fi}
      {\if@twocolumn\else\endquotation\fi}
\fi
\makeatother



\usepackage{acronym}
\usepackage{booktabs}
\usepackage{pdflscape}
\usepackage{epigraph}

\let\proof\relax
\let\endproof\relax

\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{temporal}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{xspace}
\usepackage{subcaption}
\usepackage{stmaryrd} % for short arrows
%\usepackage{parskip}  % don't indent paragraphs -- use vertical spacing instead
\usepackage[svgnames]{xcolor}  % used by preamble
\usepackage{multirow}
\usepackage{doi}   % to allow _ in doins
\usepackage{tikz}\usetikzlibrary{arrows,automata,calc,fit,positioning}
\usepackage{wrapfig}
\usepackage{booktabs}  % better tables
\usepackage{colortbl}
\usepackage{float}  % for forcing position with 'H' (like \begin{table}[H])
\usepackage{environ}  % Guarded Systems use \NewEnv to create new env for tikz pics
\usepackage{enumitem}  % Guarded Systems
\usepackage{mdframed}
\usepackage{wasysym}
\usepackage{pifont}

\usepackage{thmtools, thm-restate}

% for appendix at the end of the chapter
% + some tricks for TOC
% https://tex.stackexchange.com/questions/120716/appendix-after-each-chapter
\usepackage{appendix}
\usepackage{chngcntr}
\usepackage{etoolbox}
\AtBeginEnvironment{subappendices}{%
\chapter*{Appendix}
\addcontentsline{toc}{chapter}{~~~~Appendix}
\counterwithin{figure}{section}
\counterwithin{table}{section}
}

%%%%%%%%%%%%%% trackchanges %%%%%%%%%%%%%%
% ignore llncs note command
\let\note\relax
\let\endnote\relax

\iffinal
  \usepackage[finalold]{trackchanges} % also use \sr,\sj,\ak,\ba
\else
  \usepackage[inline]{trackchanges}
\fi

\addeditor{$A\!K$}
\addeditor{$R\!B$}
\addeditor{$S\!J$}
\newcommand{\ak}[1]{\note[$A\!K$]{#1}}
\newcommand{\rb}[1]{\note[$R\!B$]{#1}}
\newcommand{\sj}[1]{\note[$S\!J$]{#1}}
%% end of trackchanges

\usepackage{hyperref}   % goes last
\hypersetup{
    colorlinks,
    linkcolor=black,
    citecolor=black,
}

\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother

%---------------------------------------------------------------------
%---------------------------------------------------------------------
%---------------------------------------------------------------------
%---------------------------------------------------------------------
%---------------------------------------------------------------------
%---------------------------------------------------------------------


\newcommand{\mailto}[1]{\href{mailto:#1}{\nolinkurl{#1}}}
\newcommand{\ack}[1]{\smallskip\noindent\small{\textbf{Acknowledgements.} #1}}


\newcommand\abstractname{Abstract}
%\newtheorem{obs}{Observation}
%\declaretheorem[name=Theorem]{thm}
%\declaretheorem[name=Lemma]{lem}
%\declaretheorem[name=Corollary]{cor}
%\declaretheorem[name=Observation]{obs}
%\declaretheorem[name=Claim]{claim}

% BEGIN theorems
\newtheoremstyle{myexample}% name
  {5pt}%      Space above
  {5pt}%      Space below
  {}%         Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\itshape}% Thm head font
  {.}%        Punctuation after thm head
  {.5em}%     Space after thm head: " " = normal interword space;
        %       \newline = linebreak
  {}%         Thm head spec (can be left empty, meaning `normal')
{\theoremstyle{myexample} \newtheorem{example}{Example} }
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
{\theoremstyle{definition} \newtheorem{remark}{Remark} }
%\newenvironment{proof}{\begin{IEEEproof}}{\end{IEEEproof}}
%\newcommand{\qed}{}



%paragraph with some skip and bold heading
\newcommand{\parbf}[1]{\smallskip\noindent {\bf #1.}}
\newcommand{\parit}[1]{\smallskip\noindent {\it #1.}}

\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bigdotcup}{\ensuremath{\mathaccent\cdot{\bigcup}}}

\newcommand\LTL{\ensuremath{\text{LTL}}\xspace}
\newcommand\LTLmX{\ensuremath{\text{LTL}\backslash\text{X}}}
\newcommand\CTLstar{\ensuremath{{\text{CTL}^*}}\xspace}
\newcommand\CTLstarmX{\ensuremath{{\text{CTL}^*\backslash\text{X}}}\xspace}
\newcommand\CTL{\ensuremath{\text{CTL}}\xspace}

\definecolor{lightgray}{gray}{0.8}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkblue}{rgb}{0,0,.5}
\definecolor{darkred}{rgb}{0.9,0,0}
\definecolor{pink}{rgb}{0.95,0.08,0.55}
\definecolor{mygray}{gray}{.6}
\newcommand{\minor}[1]{{\footnotesize\textcolor{mygray}{#1}}}
%% end of trackchanges


%% 'such that'
\renewcommand{\|}{\mid}
%% disjoint union
\newcommand{\cupdot}{\mathbin{\dot{\cup}}}


%% specification, implication
\renewcommand{\iff}{\leftrightarrow}
\newcommand{\Iff}{\Leftrightarrow}
\newcommand{\impl}{\rightarrow}
\newcommand{\Impl}{\Rightarrow}
\newcommand{\Implied}{\Leftarrow}

% add line breaks to table cells, to labels of tikz 
% usage: \specialcellC{first line \\ second line} 
\newcommand{\specialcellC}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
\newcommand{\specialcellL}[2][c]{%
  \begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}

% temporal logic
\newcommand\G\always\xspace
\newcommand\F\eventually\xspace
\newcommand\W\weakuntil\xspace
\newcommand\U\until\xspace
\newcommand\R\releases\xspace
\newcommand\X\nextt\xspace
\newcommand\XX{\ensuremath{\nextt\!\nextt\xspace}}
\newcommand\XXX{\ensuremath{\nextt\!\nextt\!\nextt\xspace}}
\newcommand{\GF}{\G\!\F\xspace}
\newcommand{\FG}{\F\!\G\xspace}
\newcommand\E{{\ensuremath\pexists}\xspace}
\newcommand\A{{\ensuremath\pforall}\xspace}


% Latex syntax sugar
\newcommand\li{\begin{itemize}}
\newcommand\il{\end{itemize}}
\renewcommand{\-}{\item}
%\newcommand\lo{\begin{enumerate}}
%\newcommand\ol{\end{enumerate}}

\newcommand\todo[1]{\ak{\hl{todo: #1}}}

% ttfamily with bold. Use in lstslistings: 
% \begin{lstlisting}[basicstyle=\ttfamilywithbold,language=python,mathescape]
%   the code here will have bold
% \end{lstlisting}
% http://tex.stackexchange.com/questions/25249/how-do-i-use-a-particular-font-for-a-small-section-of-text-in-my-document/25251#25251
%\newcommand*{\ttfamilywithbold}{\fontfamily{lmtt}\selectfont}

\newcommand{\current}{\sethlcolor{green}\ \hl{current} \ \sethlcolor{yellow}}

\newcommand{\tpl}[1]{\left<#1\right>}

\newcommand{\edge}[3]{#1 \stackrel{{#2}}{\rightarrow} #3}
\newcommand{\trans}[1]{\stackrel{{#1}}{\rightarrow}}
\newcommand{\eqbydef}{\triangleq}

\newcommand{\I}{{2^I}}
\renewcommand{\O}{{2^O}}
\newcommand{\reach}{\mathit{rch}}
\newcommand{\rank}{\rho}
\newcommand{\RANK}{\ensuremath{R_\triangleright}\xspace}

% types of properties
\newcommand{\buchi}{B\"{u}chi\xspace}
\newcommand{\AUBW}{\ensuremath{\A(\textit{UBW})}\xspace}
\newcommand{\AUCW}{\ensuremath{\A(\textit{UCW})}\xspace}
\newcommand{\AUSW}{\ensuremath{\A(\textit{USW})}\xspace}
\newcommand{\AURW}{\ensuremath{\A(\textit{URW})}\xspace}
\newcommand{\AUXW}{\ensuremath{\A(\textit{UXW})}\xspace}

\newcommand{\ENBW}{\ensuremath{\E(\textit{NBW})}\xspace}
\newcommand{\NBW}{\ensuremath{\textit{NBW}}\xspace}
\newcommand{\AHT}{\ensuremath{\textit{AHT}}\xspace}
\newcommand{\ENCW}{\ensuremath{\E(\textit{NCW})}\xspace}
\newcommand{\ENSW}{\ensuremath{\E(\textit{NSW})}\xspace}
\newcommand{\EDSW}{\ensuremath{\E(\textit{DSW})}\xspace}
\newcommand{\ADSW}{\ensuremath{\A(\textit{DSW})}\xspace}
\newcommand{\EDRW}{\ensuremath{\E(\textit{DRW})}\xspace}
\newcommand{\EDFW}{\ensuremath{\E(\textit{DFW})}\xspace}
\newcommand{\EDBW}{\ensuremath{\E(\textit{DBW})}\xspace}
\newcommand{\ENRW}{\ensuremath{\E(\textit{NRW})}\xspace}
\newcommand{\ENXW}{\ensuremath{\E(\textit{NXW})}\xspace}

% other math macros
\newcommand{\out}{\mathit{out}}
\newcommand{\GR}{\triangleright}
\newcommand{\PhiE}{\Phi^{\GR}_\E}
\newcommand{\PhiA}{\Phi^{\GR}_\A}

\newcommand{\Inf}{\textit{Inf}}
\newcommand{\Fin}{\textit{Fin}}
\newcommand{\Pref}{\textit{Pref}}

\renewcommand{\true}{\textsf{true}\xspace}
\renewcommand{\false}{\textsf{false}\xspace}


% medium sized versions of operators
\DeclareMathOperator*{\medoplus}{\text{\raisebox{0.25ex}{\scalebox{0.8}{$\bigoplus$}}}}
\DeclareMathOperator*{\medvee}{\text{\raisebox{0.25ex}{\scalebox{0.8}{$\bigvee$}}}}
\DeclareMathOperator*{\medwedge}{\text{\raisebox{0.25ex}{\scalebox{0.8}{$\bigwedge$}}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% preamble used for pictures by tikzit
% I don't know how to import the preamble though:
% of course, you can just copy-paste it into the custom preamble,
% but the default preamble should also be changed so that tikzit can correctly display it
%    but tikzit does not allow to modify the default preamble nor to import it...

%\usepackage[svgnames]{xcolor}
\usepackage{tikz}
\usetikzlibrary{arrows,automata}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{shapes.geometric}

% for some reason,
% in this book class all fonts are larger than in the non-book version,
% so let's set font=\small
\tikzset{every picture/.style={/utils/exec={\small}}}  

\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{edgelayer,nodelayer,main}

\tikzstyle{none}=[inner sep=0pt]
\tikzset{initial text={}}

\tikzstyle{rn}=[circle,fill=White,draw=Red,minimum size=0.4cm,inner sep=0pt]
\tikzstyle{gn}=[circle,fill=White,draw=Green,minimum size=0.4cm,inner sep=0pt]
\tikzstyle{yn}=[circle,fill=White,draw=Yellow,minimum size=0.4cm,inner sep=0pt]
\tikzstyle{wn}=[circle,fill=White,draw=Black,minimum size=0.4cm,inner sep=0pt]
\tikzstyle{invisible}=[circle,fill=White,draw=White,inner sep=0pt]
\tikzstyle{textual}=[rectangle]
\tikzstyle{dot}=[circle,fill=Black,draw=Black,inner sep=0pt,minimum size=0.5mm]
\tikzstyle{uptriangle}=[regular polygon,regular polygon sides=3,shape border rotate=0,fill=Black,draw=Black,inner sep=0pt,minimum size=1mm]
\tikzstyle{text ellipse}=[rectangle,rounded corners,fill=White,draw=Black,minimum size=0.6cm,inner sep=0pt]



\tikzstyle{simple}=[-,draw=Black]
\tikzstyle{arrow}=[->,draw=Black]
\tikzstyle{dashed arrow}=[->,draw=Black,dashed]
\tikzstyle{tick}=[-,draw=Black,postaction={decorate},decoration={markings,mark=at position .5 with {\draw (0,-0.1) -- (0,0.1);}}]
\tikzstyle{ga}=[->,draw=Green]
\tikzstyle{pa}=[->,draw=DeepPink]
\tikzstyle{red}=[-,draw=Red]
\tikzstyle{pink}=[-,draw=DeepPink]
\tikzstyle{blue}=[-,draw=Blue]
\tikzstyle{green}=[-,draw=Green]
\tikzstyle{yellow}=[-,draw=DarkGoldenrod]










%%%% end of tikzit preamble
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

